Numerical stability analysis of large language models

Transformers are the state-of-the-art architecture for large language models, and a key to their scalability is the strategic usage of low-precision arithmetic. We develop a mixed-precision analysis of transformer inference, deriving bounds for the condition numbers and forward error of the architecture's constituent parts. Notably, we compare the numerical stability of LayerNorm and RMSNorm in the massive-outlier regime, tighten the error bound of softmax in the presence of attention sinks, and quantify the impact of its shifted evaluation on the sensitivity to perturbations. Furthermore, we derive novel sequence-length-independent bounds on the local Lipschitz constant of self-attention. Our worst-case error bound for transformer inference suggests that its numerical stability is determined by the interplay between weight magnitude and the growth of the residual stream. Crucially, and as validated by experiments with GPT-2, our analysis establishes that the scaling of residual-projection weights preserves the propagation of the relative rounding error unless it forces a qualitative transition in the dynamics of the residual stream.

==> preprint_maketitle.tex <==
\makeatletter

\def\@maketitle{%
  \let\footnote\thanks
  \clearemptydoublepage
    \checkoddpage\ifcpoddpage\setlength{\aboveskipchk}{-28.6pt}\else\setlength{\aboveskipchk}{-28.6pt}\fi%for checking oddpage or evenpage top skip%%
  \vspace*{\aboveskipchk}%
  \vspace{\dropfromtop}%
    \vspace*{21pt}
  \if@twocolumn\else\vspace*{-10pt}\fi
          \hbox to \textwidth{%
          \raisebox{-2pt}[0pt]{%
          }}%
    \vspace*{21pt}\par%
  %
  %\sffamilyfont
  \hbox to \textwidth{%
  \parbox[t]{\titlepagewd}{%
    \ifx\@subtitle\@empty%
    \else%
    {\sffamilyfontcn\fontsize{14}{21}\selectfont\raggedright \@subtitle \par}%
    \vspace{7.5\p@}%
    \fi%
    % Title here
        %{\fontsize{9.8bp}{10}\selectfont \MakeUppercase{\@appnotes}}\\[6.5pt]
        {\fontsize{12bp}{14pt}\selectfont\bfseries\leftskip0pt plus1fill\rightskip0pt plus1fill {\@title} \par}%%
    % Title below space
    \vspace{12\p@}%
    % Author here
        {\fontsize{10bp}{12}\selectfont\scshape\leftskip0pt plus1fill\rightskip0pt plus1fill \@author \par}%
    % Author below space
    \vspace{4\p@}
    % Address here
        %{\itshape\selectfont\leftskip0pt plus1fill\rightskip0pt plus1fill \@address \par}%
    % Address below space
    \vspace{-10\p@}
    % Correspondence author here
        {\fontsize{10bp}{12}\selectfont\leftskip0pt plus1fill\rightskip0pt plus1fill\@corresp \par}%
    % Correspondence below space
    % Editor here
    % Editor below space
    \vspace{10\p@}
    % History here
        {\fontsize{10bp}{12pt}\selectfont\leftskip0pt plus1fill\rightskip0pt plus1fill \phantom{[\@history]} \par}
    % History below space
    \vspace*{10.5pt}
    % Abstract here
    \begingroup
    \parindent=0pt
    {\fontsize{9bp}{11}\selectfont\leftskip18pt\rightskip18pt\@abstract\par}
    %\end{minipage}
    \endgroup
    %\vspace{20\p@}
    }%
  }
  %
  \vspace{13.5\p@}%
  \ifx\@boxedtext\@empty\else\vspace*{12pt}\par\fi%
  \@boxedtext
  \vspace{12\p@ plus 6\p@ minus 6\p@}%
  \vspace{\extraspace}
  \vspace*{-18pt}
}

\def\ps@opening{%
  \let\@evenhead\relax
  \let\@oddhead\relax
}

\makeatother
